Provable Statistical Rates for Consistency Diffusion Models

Diffusion models have revolutionized various application domains, including computer vision and audio generation. Despite the state-of-the-art performance, diffusion models are known for their slow sample generation due to the extensive number of steps involved. In response, consistency models have been developed to merge multiple steps in the sampling process, thereby significantly boosting the speed of sample generation without compromising quality. This paper contributes towards the first statistical theory for consistency models, formulating their training as a distribution discrepancy minimization problem. Our analysis yields statistical estimation rates based on the Wasserstein distance for consistency models, matching those of vanilla diffusion models. Additionally, our results encompass the training of consistency models through both distillation and isolation methods, demystifying their underlying advantage.

==> left.tex <==
Combining this lemma with a bound of $W_1(\bX_\varepsilon, \distri)$, the score integrated error (\cref{lemma:score}) as well as \cref{lemma: W1-TV-1}, we obtain the following results:
\begin{Lemma}
After choosing the $\beta(t)$ in \cref{eqn:vp-sde} and \cref{eqn:vp-sde-back-ode} as: $\beta(t)\asymp \frac{1}{d\log n + d^2\log(d/\varepsilon)}$ for $\forall t\in [\varepsilon, T]$, there exists a score estimator $s_\phi(\cdot, t)$ such that the consistency model $f_{\hat{\theta}}(\cdot, t)$ obtained from \cref{eqn:consistency-objective} satisfies that:
\begin{equation*}
\begin{aligned}
&\bE\left[W_1\left(f_{\hat{\theta}}(\cdot, T)_\sharp \mathcal N(0, \bm I), f_{\theta^*}(\cdot, T)_\sharp \bX_T\right)\right]\\
&~\lesssim \sqrt{d}R\exp(-\underline{\beta} T/2) + R\overline{\beta}dL\cdot \frac{T}{\sqrt{M}} + R\overline{\beta}\sqrt{d} n^{-\frac{1}{d+5}}\cdot \sqrt{\frac{TN'}{\varepsilon}} + 6RN'\cdot n^{-1/d},
\end{aligned}
\end{equation*}
which provides a Wasserstein error bound for the output distribution of $f_{\hat{\theta}}(\cdot, t)$ and $f_{\theta^*}(\cdot,t)$. Here, $R$ is the Lipschitz constraint of the optimization problem (\cref{eqn:consistency-objective}). 
\label{lemma:main1}
\end{Lemma}
